Self-Supervised Dynamic Networks for Covariate Shift Robustness

As supervised learning still dominates most AI applications, test-time performance is often unexpected. Specifically, a shift of the input covariates, caused by typical nuisances like background-noise, illumination variations or transcription errors, can lead to a significant decrease in prediction accuracy. Recently, it was shown that incorporating self-supervision can significantly improve covariate shift robustness. In this work, we propose Self-Supervised Dynamic Networks (SSDN): an input-dependent mechanism, inspired by dynamic networks, that allows a self-supervised network to predict the weights of the main network, and thus directly handle covariate shifts at test-time. We present the conceptual and empirical advantages of the proposed method on the problem of image classification under different covariate shifts, and show that it significantly outperforms comparable methods.

==> draft_sentences.tex <==
The major, now cashed, promise of this field is the ability to learn useful representations without access to human labeling.


In \cite{hendrycks2019using}, the authors propose a simple training mechanism that ties between the main task and a self-supervised task through encoder parameter sharing. 
In \cite{sun2019test}, this concept is extended to allow for an unsupervised test time adjustment of the encoder parameters (Fig. \ref{fig:hypernetworks}, left). The main insight for this approach is that the self-supervised optimization on the test sample adjusts the model for better handling the main task on that sample, thus implementing the concept of input-dependent analysis. While guaranteed in train time, the main challenge with this approach is in preserving the link between the two tasks in test time. In this work, we propose a more direct and systematic approach to this issue, that explicitly ties between the self-supervised (SS) and main task, and between the parameters $\theta$ and the input x.




relate the parameters of a self-supervised encoder
For parameter rich networks, this tempting setup can be very challenging to train \cite{bertinetto2016learning, jia2016dynamic, nachmani2019hyper}. Thus, we adopt a conservative approach that allows limited modification of the target network that is better suited for our adaptation setup and help stabilize the learning process.
\erez{This general concept gives rise to input-dependent analysis with the parameters $\theta$ now being $\theta(x)$}. In \cite{sun2019test}, input-dependency
While this approach might be tempting due to its increased flexibility, some new practical challenges might arise \cite{bertinetto2016learning, jia2016dynamic, nachmani2019hyper}. Following a theoreti 
Specifically, the effect of changing $\theta$ on the predicted label for the task $\hat{y}=F_{\theta}(x)$ is generally unexpected. Inspired by a recently proposed test-time adjustment procedure \cite{sun2019test}, we propose a training mechanism that directly controls the effect of input-driven modifications on the eventual performance of the model.\erez{further clarify the gap with previous work in this context and better specify our contribution here - perhaps unify with P6}
Our proposed input-driven adjustment is inspired by the idea  of input-dependent or dynamic-networks \cite{bertinetto2016learning, kristiadiuncertainty, nachmani2019hyper}, where the parameters of one network are determined by the output of another network on the same input. For parameter rich networks, this tempting setup can be a very challenging to train \cite{bertinetto2016learning, jia2016dynamic, nachmani2019hyper}. Thus, we adopt a conservative approach that allows limited modification of the target network that is better suited for our adaptation setup and help stabilize the learning process.


\section{Related Work}
%P5 - Related work: domain-adaptation, input-dependent hyper-networks
Our work is generally positioned within the knowledge transfer context, where numerous methodologies have been developed for extending or transferring the knowledge in the training (source) domain to some sampled test (target) domain. The different methods are typically exercised with respect to the magnitude of target domain samples available during training ($N_{target}$), and whether they are labeled for the desired task. The different approaches are summarized in Table \ref{positioninig_table}. We note that the bottom row is out of reach for common domain-adaptation techniques which are ill-posed when data is at shortage \erez{[??get citation??]}. 
The only difference between our setup and that of Online Unsupervised Domain-Adaptation (OUDA)~\cite{moon2020multi,sun2019test} is that we do not assume a common distribution between test samples. This restrictive scenario is justified either in cases where performance is critical right from the first sample of an online session or because continuity is not guaranteed, e.g. in distributed or low-frequency sensing. 
The most closely related works with respect to our experimental setup are~\cite{hendrycks2019using} where auxiliary self-supervised training proves to improve model robustness do covariate shifts demonstrated by common-corruptions, and~\cite{sun2019test} which improves upon~\cite{hendrycks2019using} by allowing test-time training of the self-supervised task. We show a significant improvement upon~\cite{sun2019test} across all types of corruptions and data-sets tested.

%Table of positioning with respect to related work
\begin{table}[t]
  \begin{center}
    \caption{Positioning}
    \label{tab:table1}
    \begin{tabular}{ccc}
      \toprule % <-- Toprule here
      \textbf{$N_{target}$} & \textbf{w/ labels} & \textbf{w/o labels}\\
      \midrule % <-- Midrule here
      $>>1$ & Transfer-Learning, DA & UDA\\
      \midrule % <-- Midrule here
      $\sim 1$ & Online Learning & OUDA, \textbf{1S-UDA}\cite{sun2019test}\\
      \bottomrule % <-- Bottomrule here
    \end{tabular}
  \end{center}
\caption{\label{positioninig_table} DA=Domain-Adaptation, U=Unsupervised, O=Online, 1S=One-Sample}
\end{table}



#### abstract

While the dominance of supervised-learning persists for most applications, the test-time performance of models is often unexpected. Specifically, it was shown how simple shifts of the input domain, known as Covariate Shifts, can lead to significant decrease of prediction accuracy. If the shifts are known during training time, robustness could be achieved using techniques like domain-adaptation or data-augmentation. However, it clear that not all possible shifts could be demonstrated or imagined during training, and a technique for achieving more general robustness is needed. Recently, it was shown how self-supervised learning along side main task learning can improve model robustness in train time, while also allowing for unsupervised adjustments in test time. In this work, we take these ideas one step further. First, we propose a method for end-to-end bridging between representations learned for self supervision to those needed for the main task. And second, we propose a simple input dependent pipeline, for directly adjusting the model to handle covariate shifts in test time. We present the conceptual and empirical advantages of the proposed methods on the problem of image classification under different covariate shifts, significantly outperforming comparable methods.
##




Thus, given a source domain, a shifted domain and a CNN with an $L$ layered convolutional encoder, we have one encoder $E_s$ trained in the source domain and $L$ encoders $\{E^{i}_t\}_{i=1}^{L}$  fine-tuned in the shifted-domain, that differ from $E_s$ only in the layer $i$. For comparing the representation similarity between each layer $i$ of the reference encoder $E_s$ and the same layer in the corresponding encoder $E^i_t$, we use the recently proposed linear-CKA index~\cite{lindsay2020convolutional}. For \emph{control}, we also run the same representation similarity experiment between corresponding layers of $E_s$ from several different random initializations. We conduct this test on the CIFAR-10-C dataset~\cite{hendrycks2019benchmarking}, with the original CIFAR-10 dataset~\cite{krizhevsky2009learning} as the source domain, and the fifteen different corrupted versions in CIFAR-10-C as different covariate shifts, resulting in fifteen different representation similarity experiments. In all experiments, we use the same 26-layer ResNet as used in \cite{sun2019test}



The problem of test-time learning is defined as a multi-task problem which utilize an self-supervised auxiliary-task in order to improve the main-task. Consider a neural network with a set of parameters $\boldsymbol{\theta}$, designed for a multi-task training, that is, a shared encoder divided into two branches. The network's parameters can be split as follows. The shared parameters, $\boldsymbol{\theta_e}$, the self-supervised task head parameters ,$\boldsymbol{\theta_s}$, and the main-task head parameters $\boldsymbol{\theta_m}$.

The main-task is defines as the following optimization problem. Given training data $(x_1,y_1),...,(x_n,y_n)$, drawn i.i.d. from a distribution $P$, i.e. the source domain, we would like to minimizing the parameters $\boldsymbol{\theta}=(\theta_1,...,\theta_L)$ of a standard $L$ layer neural network to solve the optimization problem with the loss function $l_m$:

\begin{equation}
\label{eq:main-task}
\displaystyle \min_{\boldsymbol{\theta}} \frac{1}{n} \sum_{i=1}^{n} l_m(x_i,y_i,\boldsymbol{\theta})
\end{equation}

Combining the \emph{auxiliary-task} with a loss function $l_s$ into the multi-task learning optimization problem, given the same training data from $P$, yields the joint training problem:

\begin{equation}
\label{eq:multi-task}
\displaystyle \min_{\boldsymbol{\theta_e},\boldsymbol{\theta_s},\boldsymbol{\theta_m}} \frac{1}{n} \sum_{i=1}^{n} l_m(x_i,y_i,\boldsymbol{\theta_e},\boldsymbol{\theta_m}) + 
l_m(x_i,\boldsymbol{\theta_e},\boldsymbol{\theta_s})
\end{equation}

Given this setup we can define the \emph{test-time training} optimization problem on a single test sample $x$ using the auxiliary loss:

\begin{equation}
\label{eq:test-time}
\displaystyle \min_{\boldsymbol{\theta_e}, \boldsymbol{\theta_s}} l_s(x,\boldsymbol{\theta_e},\boldsymbol{\theta_s})
\end{equation}

The test-time learning and the multi-task learning both required the loss function $l_s$ which define a specific self-supervised task. In this paper we follow up the setup of~\cite{sun2019test}, and selected the rotation prediction task~\cite{ss_rotation}. That is, rotates $x$ on the image plane by $\alpha\in\{0,90,180,270\}$ and predict the angle of rotation by a four-way classification problem. Note, that as shown in~\cite{sun2019test} other self-supervised tasks can also be used.

Upon a new test sample $x_{t+1}$, the parameters (\boldsymbol{$\theta_e$}, \boldsymbol{$\theta_s$}) are optimized again, starting from the parameters acquired by training on $P$, discarding the update made by $x_t$. 




\label{CIFAR-10-C_exp}
We start by validating the proposed methods under the CIFAR-10-C covariate shift robustness challenge defined in~\cite{hendrycks2019using}. In this challenge, all tested models are pre-trained using the original CIFAR-10 dataset. At test time, each model receives single examples from the different corruptions in CIFAR-10-C, and tested for classification accuracy.






For directly analyzing the effect of the proposed signal-dependent bridge, we examine the distribution of the $\alpha$ parameters under each of the covariate shifts in the CIFAR-10-C dataset. We train a model only on the vanilla CIFAR-10 train split, and inspect the $\alpha$ parameters of the test split and the corruption splits. Results are visualized in Fig. \ref{fig:alphas}, where we clearly see distinct clusters for almost every covariate shift. Thus, it seems that the signal-dependent bridge is able to detect the covariate shift in a completely unsupervised manner and therefore allow the encoder to adapt accordingly. Interestingly, the cluster location on the plot is a good proxy to the classification accuracy under the respective covariate-shift. For example, 'brightness' is the closest to 'original', and has the lowest test error out of the corruptions. In contrast, 'gaussian\_noise' is quite far from 'original', and has a very high test error. Moreover, when looking at the t-SNE plots of different layers, the clusters seem to behave isometrically, further suggesting that the network gains valuable and consistent covariate shift information from each sample.
of the test split and the corruption splits. Results are visualized in Fig. \ref{fig:alphas}, where we clearly see distinct clusters for almost every covariate shift. Thus, it seems that the signal-dependent bridge is able to detect the covariate shift in a completely unsupervised manner and therefore allow the encoder to adapt accordingly. Interestingly, the cluster location on the plot is a good proxy to the classification accuracy under the respective covariate-shift. For example, 'brightness' is the closest to 'original', and has the lowest test error out of the corruptions. In contrast, 'gaussian\_noise' is quite far from 'original', and has a very high test error. Moreover, when looking at the t-SNE plots of different layers, the clusters seem to behave isometrically, further suggesting that the network gains valuable and consistent covariate shift information from each sample.


Similar to ~\cite{hendrycks2019using,sun2019test}, we focus on the highly challenging scenario where we have a single test instance introducing an unknown covariate shift, nullifying the concept of a \textit{target domain}.\erez{add a sentence about OOD detection methods} Our goal is to adjust the model to be more robust under such arbitrary covariate shifts.




%%from intro
%P3 - Observations and justification
We base our method on three key hypotheses:
First, the mapping between the self-supervised encoder and the main task encoder might benefit from a data-driven optimization, rather than forcing an identity mapping through weight sharing as in~\cite{sun2019test}. 
Second, this mapping might also benefit from an input-driven adjustment, by allowing specific flexibility for each individual test instance. 
Third, sensitivity to covariate shifts might not be uniform across all layers of a deep neural network. Thus, the mapping can benefit from focusing only on specific layers.
We validate these hypotheses with corresponding empirical analysis, and show how to translate them into practical methods for significantly outperforming state-of-the-art results in covariate shift robustness for image classification~\cite{sun2019test}.



% abstract
\begin{comment}
Covariate shift is the change in the distribution of the covariates. This is normally due to test time changes in state of latent variables, which could be temporal, or spatial, or less obvious. Simple shifts of the input domain, can lead to performance degradation.
We demonstrate the power of mapping internal self-supervised representations, to those needed for a main task to overcome the covarite shift at test time. 
Given a test sample, our input-dependent model adjust its parameters in a self-supervised way, to better handle the shift.
We propose a new test time mapping which is inspired by hyper-networks, where the parameters of one network is determine by the output of another network. 
Specifically, a self-supervised encoder is dynamically control the parameters of a main task encoder -- improving the robustness to covariate shift. 
We demonstrate that our method outperforms the state of the art on the problem of image classification under different covariate shifts.

In practice, covariate-shifts are extremely common in different fields, with background-noise in speech, illumination changes in images, or transcription errors for language to name very few.

While the dominance of supervised learning persists for most applications, the test-time performance of models is often unexpected. 
%Specifically, it was shown how 
Simple shifts of the input domain, known as \emph{Covariate Shifts}, can lead to performance degradation.
%of prediction accuracy. 
Domain-adaptation or data-augmentation are often used to improve the network robustness, however it is only applicable when the shifts are known at train time \roey{a priori?}.
%If the shifts are known during training time, robustness could be achieved using techniques like domain-adaptation or data-augmentation. 
%However, not all possible shifts could be predicted, and a technique for achieving more general robustness is needed. 
To overcome this, test-time training was proposed. It utilize a single unlabeled test instance to update the model in a self-supervised way, before making the prediction on the main task. 
%Recently, it was shown how incorporating self-supervision task along with the main task, can improve robustness at train time, while also allowing for unsupervised adjustments at test time. 
In this paper, we demonstrate the power of mapping internal self-supervised representations, to those needed for the main task. We then propose an input dependent model adjustment to handle covariate shifts at test time. 
We present the conceptual and empirical advantages of the proposed methods on the problem of image classification under different covariate shifts, significantly outperforming comparable methods.

\end{comment}


%implementation details
Following section \ref{method}, and the findings in \ref{Block Sensitivity results}, we only duplicate the first group of residual blocks (G1), such that the first part of the encoder is now split into $E_s$ and $E_m$. For the data-dependent bridge (sub-sec.\ref{data_dependent_bridge}), the network has $\alpha$ parameters such that $E_m$ is not an optimizable neural network, but rather a weighted combination of $E_s$'s filters. For the input-dependent bridge \ref{signal_dependent_bridge}, the self-supervised head predicts the signal-dependent bridge parameters $\tilde{\alpha}$. 






% ---------------- ABLATION ANALYSIS -------------
% To understand the effect of bridging between $E_s$ and $E_m$ at different layers, we evaluated different versions of SSDN, where each time we use different parts of the encoder as the bridge (see Tab.~\ref{block_ablation}). While ideally bridging all layers may sound like the optimal scheme, predicting bridge parameters is less stable than vanilla backprop \tomer{does this sentence makes us sound bad?}, and therefore focusing on the encoder part with the most prominent gap (G1, see Sec.~\ref{fig:representation_similarity_freeze}) results in best performance. 


% \begin{table}[H]


% \caption{Ablation study showing the effect of bridging between different parts of the encoders.}
% \label{block_ablation}
% \centering
% \begin{tabular}{ c c c c c } 
%  \toprule
% C0 & G1 & G2 & one pass & one pass + {\small TTT}  \\ 
% \midrule 
% 0 & 0 & 1 & 30.71 & 28.69  \\ 
% 0 & 1 & 0 & \textbf{30.21} & \textbf{28.18} \\ 
% 0 & 1 & 1 & 32.16 & 30.08 \\ 
% 1 & 0 & 0 & 30.46 & 28.57 \\ 
% 1 & 0 & 1 & 33.95 & 31.64 \\ 
% 1 & 1 & 0 & 31.05 & 29.07 \\ 
% 1 & 1 & 1 & 32.53 & 30.26 \\ 
% \bottomrule

% \end{tabular}



% \end{table}
% -----------------------------------------------------


==> proposal.tex <==

\section{RESEARCH PROPOSAL}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Write your content in sections, and input them here %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Problem Definition} 

\noindent Our work lies in the intersection of two machine learning tasks: domain adaptation and continual learning. Below we briefly present each task.

\textbf{Domain Adaptation} 
In this scenario, a model is trained on labeled source data, and needs to adapt to new, unlabeled target data. The target data is correlated with the source data, but might have a significantly different distribution, or come from a completely different domain. 

\textbf{Continual Learning}
Also known as \textit{Lifelong Learning}, this task refers to a model sequentially learning new datasets, while not having access to previous learned data. The task is comprised of two opposing goals: (i) preforming well on new datasets, and (ii) retaining good performance on previously learned data.

\subsection{Motivation} 

\noindent Our motivation is two-fold:

\begin{enumerate}%[(i)]
  \item Recent advancements in the research of hypernetworks (see Sec. \ref{hyper}) offers countless 
new approaches for neural networks architectures. Hypernetworks have been proved beneficial for 2D to 3D model reconstruction~\cite{hn_gidi}, continual learning~\cite{continual_hyper}, functional image representation~\cite{hn_image}, and more~\cite{hypernetworks}. 

  \item In recent years, there have been massive efforts in the deep learning community to leverage unlabeled data, for improving supervised tasks. Labeled data is costly to acquire, whereas unlabeled data is widely available. A common approach is self-supervised learning, where a supervised model is trained using labels that could be automatically extracted from the data, without human annotation~\cite{ss_rotation, ss_color, ss_inpaint, ss_splitbrain, ss_seq, ss_sr, ss_boosting}. 
    
\end{enumerate}

We therefore propose a general framework which leverages the benefits of hypernetworks, to create a novel form of self-supervision. This unique combination has the potential to alleviate both domain adaptation tasks and continual learning scenarios, in a unified architecture.



\subsection{Challenge} 
% Below we present the distinct challenges characterizing the two tasks related to our work.
    
In \textbf{Domain Adaptation}, we train a model on a source domain data, where usually a large labeled dataset is available (e.g. synthetic driving footage), and later adapt the model to a target dataset (e.g. real driving videos). Robustly transferring performance on the source data, to the unlabeled target data, isn't trivial. Specifically, we cannot assume learned features of the source data will reliably represent the target data.


% a model is trained on labeled source data, and tested on different target data. Due to the different distributions of train and test data, a model will almost always suffer from degraded performance at test time. 
% Potentially, every real-world machine learning model could benefit from good domain adaptation in the test phase, but
% Since we can never predict the test data distribution, an optimal domain adaptation solution is basically out of reach.
% Domain adaptation depicts a training challenge as well. In a shortage of labeled target domain data, it is common to 


% at learning a robust model with good performance on both source and target datasets, even if their distributions highly differ.


In \textbf{Continual Learning}, we wish to retain good performance on out-of-reach data, while also improving performance new datasets. Na\"ive approaches, such as fine-tuning, usually results in degraded performance over previously seen data. This happens since the model doesn't have access to the old labels, and we only optimize for the new dataset. Moreover, even in a hypothetical case where all datasets are available, retaining good performance on different domains requires large, memory consuming networks. 


\subsection{Previous related works}


\textbf{Domain Adaptation}
Most approaches to domain adaptation focused on learning domain invariant features~\cite{deep_domain_conf, deep_coral, ganin2015, ganin2017}. Kang \textit{et al.}~\cite{contrastive_adaptation} achieved state-of-the-art results by introducing a contrastive domain discrepancy approach, minimizing intra-class domain discrepancy, while maximizing the inter-class discrepancy. Xu \textit{et al.}~\cite{ssda} showed that simple self-supervised pretext tasks are highly effective for domain adaptation. In our work, we also leverage this insight, but use a more sophisticated form of self-supervision.

\textbf{Continual Learning}
Much work has been done to alleviate the forgetting of deep neural networks. Oquab \textit{et al.}~\cite{finetuning} simply froze early network layers, while fine-tuning later layers on target data. Other approaches aimed at creating networks with modules or pathways that specialized in certain tasks~\cite{expert_gate, pathnet}. Another line of works used a regularization scheme to bias for old network weights over new ones~\cite{forgetting_ian2014, forgetting_2017, synaptic}. 

\textbf{Self-Supervision}
Many self-supervision works aimed at learning meaningful domain features through image generation tasks, such as colorization~\cite{ss_color}, inpainting~\cite{ss_inpaint}, super-resolution~\cite{ss_sr} and cross-channel prediction~\cite{ss_splitbrain}. Other pretext tasks focused on context understanding. For example, solving jigsaw puzzles~\cite{jigsaw}, rotation angle prediction~\cite{ss_rotation}, and frame sequence understanding~\cite{ss_seq}. In~\cite{ss_boosting}, a knowledge transfer approach is taken, decoupling the model of the self-supervised network, from the main task model. Our method also employs a separate network for  self-supervision, but rather than use it as a teacher for knowledge distillation, we use it as a hypernetwork predicting the weights of the main task network.

\textbf{HyperNetworks}
Ha \textit{et al.}~\cite{hypernetworks} used hypernetworks for sequence modelling tasks. Bertinetto \textit{et al.}~\cite{hn_oneshot} predicted network weights from a single exemplar image. More recently, Littwin \textit{et al.}~\cite{hn_gidi} used hypernetworks for estimating a 3D model given a 2D image. Highly related to our approach is the work of von Oswald \textit{et al.}~\cite{continual_hyper}. Their method employs hypernetworks to obtain task-conditioned networks, which are used to "remember" task-related weights. However, this approach uses the explicit input of a task embedding, while our architecture implicitly learns network weights, conditioned on a single image. Moreover, our framework inherently integrates self-supervision, which makes it appropriate not only for continual learning, but also for domain adaptation. 

ADD THIS: functional image representation~\cite{hn_image}
Bayesian inference \cite{hn_bayesian}

\subsection{General description of the proposed method}

\subsection{HyperNetworks} \label{hyper}
\noindent Hypernetworks are neural networks that predict weights for other networks. As shown in Fig. \ref{fig:hypernetworks}, $f$ is a network predicting the weights of the network $g$. The networks can either receive two different inputs, or the same one.


\subsection{Self-Supervised HyperNetworks}

\noindent The main idea of this research is using hypernetworks as self-supervised feature extraction modules, while at the same time predicting the weights of a network solving the main task. Our approach is general and adaptable to many domains. For the purpose of illustration and validation, we will focus on computer vision tasks. 

Let $\{f_i\}_{i=1}^N$ be $N$ neural networks, and $x$ be an input image. Every network $f_i$ preforms some self-supervised task with respect to $x$, such as: rotation angle prediction~\cite{ssda}, solving jigsaw puzzles~\cite{jigsaw}, colorization~\cite{colorization}, inpainting~\cite{inpainting}, and more. In addition, each network $f_i$ also outputs a vector $w_i$. All $w_i$ vectors are the input of a network $W$, which outputs the weights $\theta_x$ of a network $g(\theta_x)$. The network $g$ receives $x$ as an input and preforms the main task at hand (i.e. classification, segmentation, etc.). All in all, we have: $ g(x; \theta_x) = g(x; W({\{f_i(x)\}}_{i=1}^N))$. 

In other words, ${\{f_i\}}_{i=1}^N$ and $W$ are hypernetworks predicting the weights of the main network $g$, conditioned on the input image $x$.
% That is: 
% \centering
% $y = g(x; \theta_x) = g(x; W({f_i}_{i=1}(x)^N)) $ 
This approach combines the powerful capabilities of hypernetworks with the concept of self-supervision: hypernetworks can efficiently represent a massive diversity of main task networks $g$, while self-supervision allows the conditioning on an input image to parameterize $g$ in an optimized manner. 

There are many potential training / testing regimes for this kind of architecture. Here we propose two training regimes, each accounts for a different task. 

\begin{enumerate}%[(i)]

\item \textbf{Domain adaptation tasks}
Optimize over ${\{f_i\}}_{i=1}^N$ with the goal of minimizing the self-supervised loss. After $K$ steps, or after the loss is under a certain threshold, pass $x$ through $W$ and $g$, and optimize for the main task loss. When training on target data, optimize for the self-supervised loss for $K'$ steps, and pass $x$ through $g$ using the last acquired weights $w_i$. 
    
\item \textbf{Continual learning tasks}
Optimize over all networks in one pass, with the goal of minimizing the self-supervised loss and the main task loss at once. 

\end{enumerate}

A key element of this research is not only exploring the appropriate architectures for this framework, but also finding the right training regime for each task. Due to the different goals of domain adaptation and continual learning, there might be different optimal training regimes for each task. Nevertheless, we would also aim to find a unified training and architecture framework to perform well on both tasks. 


\subsection{Novelty}
\noindent Our contributions are three-fold:

\begin{enumerate}
    \item We propose the first framework combining hypernetworks with self-supervision, and validate its efficacy.
    \item Our solution is the first to use hypernetworks for domain adaptation.
    \item Our framework accounts for two machine learning tasks at once: domain adaptation and continual learning. 
\end{enumerate}
